Detecting Harmful Online Conversational Content towards LGBTQIA+ Individuals

Online discussions, panels, talk page edits, etc., often contain harmful conversational content i.e., hate speech, death threats and offensive language, especially towards certain demographic groups. For example, individuals who identify as members of the LGBTQIA+ community and/or BIPOC (Black, Indigenous, People of Color) are at higher risk for abuse and harassment online. In this work, we first introduce a real-world dataset that will enable us to study and understand harmful online conversational content. Then, we conduct several exploratory data analysis experiments to gain deeper insights from the dataset. We later describe our approach for detecting harmful online Anti-LGBTQIA+ conversational content, and finally, we implement two baseline machine learning models (i.e., Support Vector Machine and Logistic Regression), and fine-tune 3 pre-trained large language models (BERT, RoBERTa, and HateBERT). Our findings verify that large language models can achieve very promising performance on detecting online Anti-LGBTQIA+ conversational content detection tasks.

==> 06related.tex <==
\section{Related Work}\label{sec:related}

Several works have been proposed for the task of harmful content detection such as gender bias, toxicity, offensiveness, abusiveness, and hate speech on social media (see \citet{fortuna-etal-2020-toxic} for definitions). Starting with one of the most popular social media platforms, Twitter \cite{Founta_2018, nejadgholi-cross, waseem-etal-2017-understanding, fortuna-etal-2020-toxic, 10.1145/3442188.3445875, razo-kubler-2020-investigating, zampieri-etal-2019-semeval, waseem-hovy-2016-hateful}, or other social media platforms, such as Reddit \cite{razo-kubler-2020-investigating, wang-etal-2020-detect, zampieri-etal-2019-semeval}, Facebook \cite{glavas-etal-2020-xhate, zampieri-etal-2019-semeval}, Whatsapp \cite{10.1145/3442381.3450137}. 

Works have also attempt to tackle this problem exploiting data from other online conversational platforms such as news media \cite{10.1145/3442442.3452325, razo-kubler-2020-investigating, zampieri-etal-2019-semeval}, Wikipedia discussions/talk page edits and bios \cite{10.1145/3485447.3512134, fortuna-etal-2020-toxic, glavas-etal-2020-xhate, nejadgholi-cross}, and online discussion forums and chatrooms \cite{wang-etal-2020-detect, gao-etal-2020-offensive}.

Over the past years, there has been an increased focus on addressing societal bias issues related to language around gender \cite{zmigrod-etal-2019-counterfactual, 10.1145/3442442.3452325, rudinger-etal-2018-gender, DBLP:journals/corr/abs-1910-10486} and racial bias \cite{davidson-etal-2019-racial, DBLP:journals/corr/BlodgettO17, DBLP:journals/corr/abs-2005-12246, DBLP:journals/corr/abs-1910-10486}. Meanwhile, there has been relatively little work on societal bias such as toxicity, offensive and abusive language, and hate speech detection for LGBTQIA+ individuals \cite{DBLP:journals/corr/abs-2109-00227}. Recently, NLP researchers are narrowing their focused work to detect and measure online harmfulness against LGBTQIA+ individuals \cite{barikeri-etal-2021-redditbias, DBLP:journals/corr/abs-2109-00227}. Specifically, \citet{DBLP:journals/corr/abs-2109-00227} provides a new hierarchical taxonomy for online homophobia and transphobia detection, as well as an homophobic/transphobic labeled dataset which comprises 15,141 annotated multilingual Youtube comments.









==> 07conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this study, we conducted a systemic evaluation of harmful comments geared towards the LGBTQIA+ community by real Reddit users by isolating and labeling the queerness (\textit{LGBTQIA+}, \textit{straight}) dimension from \textsc{RedditBias} \cite{barikeri-etal-2021-redditbias}. We exploit two out-of-the-box ML methods and 3 state-of-the-art large language models to evaluate the harmfulness of comments and our findings show promising results. 

Despite HateBERT \cite{DBLP:journals/corr/abs-2010-12472} being pre-trained for hate speech and abusive language detection, BERT outperformed all our proposed baseline models and LLMs achieving an F1-score $\geq$ 0.82 for each label, with the exception of the $\mathsf{threat}$ (Th) label due to the extremely low number of \textit{harmful} samples in our multi-label classification task. While this dataset may be useful to understand societal biases, we must warrant mentioning that examples containing \textit{stereotypes}, \textit{profanity}, \textit{vulgarity} and other harmful language that were categorized into 6 distinct classes may be more offensive, triggering or disturbing than the numbers reflected in both the paper and dataset to LGBTQIA+ individuals.

We intend to release our multi-labeled dataset for future shared tasks of online Anti-LGTBQIA+ content detection. We hope that our contributions can constitute potential groundwork on ways that LGBTQIA+ relevant data can effectively be integrated in conversational platforms (e.g., Reddit, Twitter, Facebook) to better facilitate harmful online conversational content. In the future, we aim to explore bias mitigation solutions towards members of the LGBTQIA+ community with the objective of creating a safe and inclusive place that welcomes, supports, and values all LGBTQIA+ individuals, activists and allies both online and offline.





